ExpertLongBench: Benchmarking Language Models on Expert-Level Long-Form Generation Tasks with Structured Checklists

This paper introduces ExpertLongBench, an expert-level benchmark containing 11 tasks from 9 domains that reflect realistic expert workflows and applications. Beyond question answering, the application-driven tasks in ExpertLongBench demand long-form outputs that can exceed 5,000 tokens and strict adherence to domain-specific requirements. Notably, each task in ExpertLongBench includes a rubric, designed or validated by domain experts, to specify task requirements and guide output evaluation. Furthermore, we propose CLEAR, an evaluation framework that supports accurate evaluation of long-form model outputs in our benchmark. To achieve fine-grained, expert-aligned evaluation, CLEAR derives checklists from both model outputs and references by extracting information corresponding to items in the task-specific rubric. Checklist items of model outputs are then compared with corresponding items of reference outputs to assess their correctness, enabling grounded evaluation. We benchmark 13 popular large language models (LLMs) and analyze components in CLEAR, showing that (1) existing LLMs, with the top performer Gemini-2.5-Pro achieving only a 33.4 F1 score, require significant improvement for expert-level tasks; (2) models can generate content corresponding to the required aspects, but far from correct; and (3) accurate checklist extraction and comparison in CLEAR can be achieved by open-weight models for more scalable, reproducible, and low-cost usage.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> sections/backup/01.tex <==
\section{Introduction} 



% introducing expert-level tasks
Large Language Models (LLMs) have demonstrated strong capabilities in performing everyday general-purpose tasks such as answering general knowledge questions, writing emails, and summarizing texts \cite{chowdhery2023palm,achiam2023gpt,touvron2023llama}. 
As LLMs become increasingly integrated into high-stake and domain-specific fields of daily life such as healthcare, legal analysis, and scientific research \cite{shaheen2021applications,cascella2023evaluating,siino2025exploring,ifargan2025autonomous,si2024can}, a critical question arises: can they reliably support tasks that require expert-level knowledge and reasoning?
We define expert-level tasks as domain-specific tasks that require a certain level of education for successful completion.
Successfully enabling LLMs to perform such tasks can accelerate domain-specific workflows, enhance decision-making, and unlock broader, high-impact applications across professional fields. 
% significance of reliably evaluate expert-level tasks
As such, developing benchmarks and establishing more reliable evaluation practices that better reflect real-world expert demands to assess LLMs' capability on solving expert-level task is important. 


Previous efforts to evaluate LLMs' expert-level capabilities have primarily fallen into two categories.
The first category uses proxy tasks such as multiple-choice or exam-style questions, as represented by MMLU \cite{hendrycks2020measuring}, AGIEval \cite{zhong2023agieval}, MMLU-Pro \cite{wang2024mmlu} and GPQA \cite{rein2024gpqa}. % HLE
While these benchmarks provide a basic measure of model accuracy, they merely indicate whether the model is correct or incorrect, offering little insight into why it fails or how it can improve. Moreover, they do not reflect how humans use LMs in practice by oversimplifying expert tasks to short-form, classification-based, or exam-style questions, which resemble academic tests rather than real-world professional challenges.
Consequently, they fall short of systematically capturing the complexity of real-world tasks and rigorous professional standards that real-world expert tasks demand, overlook the practical needs of expert domain, and neglect the essential focus on expert-level task-solving capabilities that are essential for real-world applications.
The second category focuses on generation tasks that evaluate models' ability to answer specialized information-seeking questions, such as ExpertQA \cite{malaviya2023expertqa}.
The short-form or closed-ended nature of input in both types of benchmarks fundamentally limits their ability to effectively assess critical skills essential for expert-level tasks. This design constraint prevents models from demonstrating contextual comprehension, which involves accurately understanding implicit and domain-specific information within a given context; information organization and integration, which requires synthesizing and structuring complex data from multiple sources; and complex articulation, which demands the clear, coherent, and accurate presentation of detailed explanations. High performance on these narrowly designed tasks does not necessarily imply the ability to succeed on real-world tasks, highlighting the risk of overlooking the broader capabilities required in practice \cite{brown2020language, wu2025towards, kim2024biggen}.
Previous evaluations further adopt coarse-grained measures like overall “helpfulness” scores to evaluate model competence  \cite{malaviya2023expertqa,li2023alpacaeval,zheng2023judging,chan2023chateval,liu2023g}. However, perceptions of coarse-grained evaluation rubrics can vary from person to person \cite{kim2024biggen}. Evaluation rubrics are crucial for ensuring that assessments are conducted reliably. Without a well-designed objective rubric, the reliability and reproducibility of evaluation results cannot be guaranteed.


To address these limitations, we introduce \textbf{\benchmark}, a long-form, expert-level, multi-disciplinary benchmark accompanied by checklist-based fine-grained evaluation rubrics that better reflect real-world expert demands and adopt a decomposed-based automatic evaluation method to evaluate LLM performance on these tasks. 
Specifically, our benchmark spans 12 expert-level tasks across 9 diverse domains, accommodating a wide range of input lengths.
These domains encompass law, material science, education, healthcare, chemistry, biology, medicine, environment, social and governance (ESG), and cybersecurity. 
\benchmark is designed to be a living resource that evolves over time, ensuring its continued relevance and alignment with evolving expert practices. To achieve this, we plan to expand the benchmark through a dynamic, community-driven approach. Specifically, our research team will regularly review developments in expert domains, identifying emerging challenges and adapting them into new benchmark tasks. 
At the same time, we actively encourage contributions from the research community, including proposing new tasks, suggesting iterative improvements to existing tasks, and providing domain-specific insights. Submitted tasks will undergo a rigorous review process to ensure quality and alignment with the objectives to evaluate LMs' capability on solving expert-level tasks.
By maintaining this dynamic, community-driven approach, \benchmark will continue to grow and stay current with the latest advancements in expert domains.

Unlike prior benchmarks, as summarized in Table \ref{tab:benchmark_comparison}, \benchmark rigorously evaluates models across a comprehensive range of 11 critical competencies, including knowledge memorization, knowledge understanding, knowledge application, and knowledge creation, as well as reasoning, planing, contextual comprehension, information organization, information aggregation and integration, complex task-solving, and complex information articulation. In contrast, existing benchmarks are restricted to assessing a limited subset of these essential skills, providing an incomplete picture of model proficiency in expert-level contexts. Detailed capability subset accessed by existing benchmarks are discussed in the Appendix. 

However, determining whether an output is "good" remains challenging due to the inherently subjective nature of long-form evaluation.
Drawing inspiration from human studies that emphasize the critical role of precise evaluation criteria in conducting effective interviews \cite{cannell1981research, machado2003qualitative}, we design \textbf{CLEAR}, \textbf{C}heck\textbf{L}ist-based \textbf{E}xpert-level task \textbf{A}ssessment \textbf{R}ubrics for each task that better align with real-world expert needs.
These fine-grained checklist-based rubrics enable nuanced evaluation of model outputs on complex expert-level tasks. To facilitate scalable evaluation, we further adopt a decomposition-based automatic evaluation method for assessing LLM performance across complex, high-stake expert scenarios\footnote{The benchmark, evaluation checklists, detailed resource of evaluation method will all be released.}.

We evaluate 12 large language models on the proposed benchmark. Our key findings are summarized as follows: [TBD].


\begin{table}[htbp] 
\centering
\small
\begin{tabularx}{0.9\textwidth}
{ccccc}
\toprule
\textbf{Benchmark} & \textbf{Output Form} &  \textbf{Topics}  & \textbf{Capability Set}\\ \toprule
% \hline
MMLU \cite{hendrycks2020measuring} & Multi-choice & Domain-specific & Subset\\
AGIEval \cite{zhong2023agieval} & Multi-choice & Domain-specific & Subset\\
GPQA \cite{rein2024gpqa} & Multi-choice & Domain-specific & Subset \\
% \hline
HLE \cite{phan2025humanity} & Short-form & Domain-specific & Subset\\
ExpertQA \cite{malaviya2023expertqa} & Short-form & Domain-specific & Subset\\
WildBench \cite{lin2024wildbench}& Short-form & Common & Subset
\\
BIGGEN BENCH \cite{kim2024biggen} & Long-form & Common & Subset\\
\textbf{\benchmark (ours)} & Long-form & Domain-specific &  All
\\
\bottomrule
% column 1: multi-choice short-form (merge authentic and long-form and open ended, HLE - short form)
% column 2: domain-application based [specific term]
\end{tabularx}
\caption{
Comparison between our benchmark and existing benchmarks. }
\label{tab:benchmark_comparison}
\end{table}




%% version 2
{
% % introducing expert-level tasks
% Large Language Models (LLMs) have demonstrated strong capabilities in performing everyday general-purpose tasks such as answering general knowledge questions, writing emails, and summarizing texts \cite{chowdhery2023palm,achiam2023gpt,touvron2023llama}. 
% As LLMs become increasingly integrated into high-stake and domain-specific fields of daily life such as healthcare, legal analysis, and scientific research \cite{shaheen2021applications,cascella2023evaluating,siino2025exploring,ifargan2025autonomous,si2024can}, a critical question arises: can they reliably support tasks that require expert-level knowledge and reasoning?
% We define expert-level tasks as domain-specific tasks that require a certain level of education for successful completion.
% % We define expert-level tasks as tasks that require specialized domain knowledge, complex reasoning, and adherence to professional norms that are typically expected of trained human experts. \shuyang{i think the definition is vague, but not sure how to better define, domain-specific is good but need to train graduate stu to do}
% % significance of addressing expert-level tasks
% Successfully enabling LLMs to perform such tasks can accelerate domain-specific workflows, enhance decision-making, and unlock broader, high-impact applications across professional fields.
% % Successfully addressing expert-level tasks implies not only technical sophistication but also economic and societal consequences, as such systems may begin to meet the substitution threshold for expert human labor. This transition carries profound economic and societal implications, including the restructuring of industries, large-scale workforce transformations, and a fundamental redefinition of human-AI collaboration. 
% % significance of reliably evaluate expert-level tasks
% As such, developing benchmarks and establishing more reliable evaluation practices that better reflect real-world expert demands to assess LLMs' capability on solving expert-level task is important. 


% % significance and challenge of reliably evaluate LLMs' capability on expert-level tasks
% % \lu{this para doesn't echo with our contributions, e.g. what's missing from existing design of expert-level benchmarks (there is MMLU; short form, not reflecting how human uses LMs), why long-form, why checklist-based evaluation. can just directl write the next paragraph on `previois efforts...'}
% % Yet reliably evaluating LLMs' proficiency in expert-level domains remains a formidable challenge. 
% % Unlike general applications, expert domains impose substantially higher demands on factual precision, domain-specific reasoning, and adherence to professional standards, where inaccuracies can result in significant real-world consequences. 
% % Thus, evaluating LLMs’ proficiency in expert-level tasks requires benchmarks that reflect the complexity and stakes of professional practice. Moreover, rigorous and objective evaluation is essential not only to accurately assess models' capabilities on solving expert-level tasks, but also to identify critical limitations, guide model improvement, and ensure the responsible use of LLMs in high-stakes scenarios. \jie{too long}

% % \lu{this para can be strengthened with how each type of design is problematic}
% Previous efforts to evaluate LLMs' expert-level capabilities have primarily fallen into two categories.
% The first category uses proxy tasks such as multiple-choice or exam-style questions, as represented by MMLU \cite{hendrycks2020measuring}, AGIEval \cite{zhong2023agieval}, MMLU-Pro \cite{wang2024mmlu} and GPQA \cite{rein2024gpqa}. % HLE
% While these benchmarks provide a basic measure of model accuracy, they merely indicate whether the model is correct or incorrect, offering little insight into why it fails or how it can improve. Moreover, they do not reflect how humans use LMs in practice by oversimplifying expert tasks to short-form, classification-based, or exam-style questions, which resemble academic tests rather than real-world professional challenges.
% Consequently, they fall short of systematically capturing the complexity of real-world tasks and rigorous professional standards that real-world expert tasks demand, overlook the practical needs of expert domain, and neglect the essential focus on expert-level task-solving capabilities that are essential for real-world applications.
% The second category focuses on generation tasks that evaluate models' ability to answer specialized information-seeking questions, such as ExpertQA \cite{malaviya2023expertqa}.
% The short-form or closed-ended nature of input in both types of benchmarks fundamentally limits their ability to effectively assess critical skills essential for expert-level tasks. This design constraint prevents models from demonstrating contextual comprehension, which involves accurately understanding nuanced and domain-specific information within a given context; information organization and integration, which requires synthesizing and structuring complex data from multiple sources; and complex articulation, which demands the clear, coherent, and accurate presentation of detailed explanations. High performance on these narrowly designed tasks does not necessarily imply the ability to succeed on real-world tasks, highlighting the risk of overlooking the broader capabilities required in practice \cite{brown2020language, wu2025towards, kim2024biggen}.
% Previous evaluations further adopt coarse-grained measures like overall “helpfulness” scores to evaluate model competence  \cite{malaviya2023expertqa,li2023alpacaeval,zheng2023judging,chan2023chateval,liu2023g}. However, perceptions of coarse-grained evaluation rubrics can vary from person to person \cite{kim2024biggen}. Evaluation rubrics are crucial for ensuring that assessments are conducted reliably. Without a well-designed objective rubric, the reliability and reproducibility of evaluation results cannot be guaranteed.
% % While these benchmarks have provided valuable initial insights, they often oversimplify expert tasks to short-form, classification-based, or exam-like problems, resembling academic tests rather than real-world professional tasks. 
% % Consequently, they fall short of systematically capturing the complexity of real-world tasks and rigorous professional standards that real-world expert tasks demand, overlook the practical needs of expert domain, and neglect the essential focus on expert-level task-solving capabilities that are essential for real-world applications.
% % Moreover, perceptions of coarse-grained evaluation rubrics can vary from person to person \cite{kim2024biggen}. Evaluation rubrics are crucial for ensuring that assessments are conducted reliably. However, when papers fail to design objective rubric, there is no guarantee of the reliability and reproducibility of their evaluation results.
% % \lu{previous 3 paragraphs can be merged, highlighting the need of long-form responses tasks and evaluation methods}\jie{think about how to highlight the importance of long-form responses tasks}

% To address these limitations, we introduce \textbf{\benchmark}, a long-form, expert-level, multi-disciplinary benchmark accompanied by checklist-based fine-grained evaluation rubrics that better reflect real-world expert demands and adopt a decomposed-based automatic evaluation method to evaluate LLM performance on these tasks. 
% Specifically, our benchmark spans 12 expert-level tasks across 9 diverse domains, accommodating a wide range of input lengths.
% These domains encompass law, material science, education, healthcare, chemistry, biology, medicine, environment, social and governance (ESG), and cybersecurity. 
% Our benchmark is designed to be a living resource that evolves over time, ensuring its continued relevance and alignment with evolving expert practices. To achieve this, we plan to expand the benchmark through a dynamic, community-driven approach. Specifically, our research team will regularly review developments in expert domains, identifying emerging challenges and adapting them into new benchmark tasks. 
% At the same time, we actively encourage contributions from the research community, including proposing new tasks, suggesting iterative improvements to existing tasks, and providing domain-specific insights. Submitted tasks will undergo a rigorous review process to ensure quality and alignment with the objectives to evaluate LMs' capability on solving expert-level tasks.
% By maintaining this dynamic, community-driven approach, our benchmark will continue to grow and stay current with the latest advancements in expert domains.

% Unlike prior benchmarks, as summarized in Table \ref{tab:benchmark_comparison}, \benchmark rigorously evaluates models across a comprehensive range of 11 critical competencies, including knowledge memorization, knowledge understanding, knowledge application, and knowledge creation\jie{creation to be confirmed}, as well as reasoning, planing, contextual comprehension, information organization, information aggregation and integration, complex task-solving\jie{no sure whether problem-solving is more suitable}, and complex information articulation. In contrast, existing benchmarks are restricted to assessing a limited subset of these essential skills, providing an incomplete picture of model proficiency in expert-level contexts.
% % Unlike prior benchmarks, as summarized in Table \ref{tab:benchmark_comparison}, our tasks focus on real-user data, open-ended long-form generation, and task-solving capabilities targeting expert-level applications. These tasks are motivated by real-world expert needs and go beyond simple multiple-choice or knowledge-querying questions.
% % These tasks are grounded in realistic professional scenarios that require planning, reasoning, synthesis, justification, and domain reasoning—capabilities essential for Expert AGI. % after failure model analysis 

% % \lu{create a new para for checklist-based fine-grained evaluation}
% However, determining whether an output is "good" remains challenging due to the inherently subjective nature of long-form evaluation.
% Drawing inspiration from human studies that emphasize the critical role of precise evaluation criteria in conducting effective interviews \cite{cannell1981research, machado2003qualitative}, we design \textbf{CLEAR}, \textbf{C}heck\textbf{L}ist-based \textbf{E}xpert-level task \textbf{A}ssessment \textbf{R}ubrics for each task that better align with real-world expert needs.
% These fine-grained checklist-based rubrics enable nuanced evaluation of model outputs on complex expert-level tasks. To facilitate scalable evaluation, we further adopt a decomposition-based automatic evaluation method for assessing LLM performance across complex, high-stake expert scenarios\footnote{The benchmark, evaluation checklists, detailed resource of evaluation method will all be released.}.

% We evaluate 12 large language models on the proposed benchmark. Our key findings are summarized as follows: [TBD].
% % In addition, we assess the reliability of existing LLM-as-a-judge methods in evaluating expert-level tasks, providing insights into their strengths and limitations in high-stakes, open-ended scenarios.

% \begin{table}[htbp] 
% \centering
% \small
% \begin{tabularx}{\textwidth}
% {ccccc}
% \toprule
% \textbf{Benchmark} & \textbf{Output Form} &  \textbf{Topics} & \textbf{Application-Driven?} & \textbf{Capability Set}\\ \toprule
% % \hline
% MMLU \cite{hendrycks2020measuring} & Multi-choice & Domain-specific & Exam question& Subset\\
% AGIEval \cite{zhong2023agieval} & Multi-choice & Domain-specific & Exam question& Subset\\
% GPQA \cite{rein2024gpqa} & Multi-choice & Domain-specific & & Subset \\
% % \hline
% HLE \cite{phan2025humanity} & Short-form & Domain-specific & & Subset\\
% ExpertQA \cite{malaviya2023expertqa} & \jie{Short-form?} & Domain-specific & & Subset\\
% WildBench \cite{lin2024wildbench}& \jie{Short-form?} & Common & & Subset
% \\
% BIGGEN BENCH \cite{kim2024biggen} & \jie{Long-form?} & Common & & Subset\\
% \textbf{\benchmark (ours)} & Long-form & Domain-specific & &  All
% \\
% \bottomrule
% % column 1: multi-choice short-form (merge authentic and long-form and open ended, HLE - short form)
% % column 2: domain-application based [specific term]
% \end{tabularx}
% \caption{
% Comparison between our benchmark and existing benchmarks. }
% \label{tab:benchmark_comparison}
% \end{table}


% \begin{table}[htbp] 
% \centering
% \small
% \begin{tabularx}{\textwidth}
% {cccc>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{2.5cm}}
% \toprule
% \textbf{Benchmark} & \textbf{Authentic} & \textbf{Open-Ended} & \textbf{Long-Form} & \textbf{Real-World Task Solving} & \textbf{Tasks Motivated from Expert Needs}  \\ \toprule
% % \hline
% MMLU \cite{hendrycks2020measuring} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}}& \cellcolor{white}\textcolor{red}{\ding{55}}& \cellcolor{white}\textcolor{red}{\ding{55}} \\
% MMLU-Pro \cite{wang2024mmlu} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}}& \cellcolor{white}\textcolor{red}{\ding{55}}& \cellcolor{white}\textcolor{red}{\ding{55}}\\
% % \hline
% AGIEval \cite{zhong2023agieval} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}}\\
% GPQA \cite{rein2024gpqa} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{green}{\checkmark} \jie{(expert create hard exam-like question)}  \\
% % \hline
% HLE \cite{phan2025humanity} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{green}{\checkmark} &
% \cellcolor{white}\textcolor{red}{\ding{55}} &
% \cellcolor{white}\textcolor{red}{\ding{55}} &
% \cellcolor{white}\textcolor{red}{\ding{55}}\\
% % \hline
% % \hline
% % OpenAGI \cite{ge2023openagi} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{red}{\ding{55}} \\
% % \hline

% ExpertQA \cite{malaviya2023expertqa} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{red}{\ding{55}} & \cellcolor{white}\textcolor{green}{\checkmark}\\
% WildBench \cite{lin2024wildbench}& 
% \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{red}{\ding{55}}\\
% \textbf{\benchmark (ours)} & 
% \cellcolor{white} \textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark} & \cellcolor{white}\textcolor{green}{\checkmark}\\
% \bottomrule
% % column 1: multi-choice short-form (merge authentic and long-form and open ended, HLE - short form)
% % column 2: domain-application based [specific term]
% \end{tabularx}
% \caption{\lu{do we need both mmlu and mmlu-pro? adding BIGGEN BENCH}
% Comparison between our benchmark and existing benchmarks. \emph{Authentic} indicates that the data originates from real user requests.\jie{Is 'RealUser' a more suitable word here?} \emph{Open-Ended} and \emph{Long-Form} refers to free-form and long model outputs. \emph{Real-World Task Solving} shows data for evaluating practical task-solving ability. \emph{Tasks Motivated by Expert Needs} signifies that the tasks are inspired by the actual needs of domain experts.}
% \label{tab:benchmark_comparison}
% \end{table}
}




%% version 1
{
% The accelerating capabilities of large language models (LLMs) \cite{chowdhery2023palm,achiam2023gpt,touvron2023llama} have reignited global discourse surrounding artificial general intelligence (AGI)—a concept typically reserved for systems that match or exceed human-level performance across a wide range of tasks \cite{bubeck2023sparks,y2023artificial,ge2023openagi,latif2023artificial,mialon2023gaia}. Despite growing attention, meaningful discussions around AGI remain hindered by the absence of precise, actionable definitions. To address this gap, 
% Morris et al. \cite{morris2023levels} proposed a structured taxonomy that frames AGI development along two axes: generality (task breadth) and performance (task depth). Within this framework, Level 3—referred to as \textbf{Expert AGI}—is defined as an AI system that performs at or above the 90th percentile of skilled human adults across a broad range of tasks. 
% Reaching this level implies not only technical sophistication but also economic and societal consequences, as such systems may begin to meet the substitution threshold for expert human labor. This transition could profoundly reshape industries, trigger large-scale workforce shifts, and redefine human-AI collaboration. 
% As such, developing benchmarks that better reflect real-world expert demands to assess the emergence of Expert AGI is not only a technical necessity, but a societal imperative.

% Existing expert-level AGI benchmarks (e.g., MMLU \cite{hendrycks2020measuring}, AGIEval \cite{zhong2023agieval}, ExpertQA \cite{malaviya2023expertqa}, MMMU \cite{yue2024mmmu}, and the recent HLE \cite{phan2025humanity}) exhibit several fundamental shortcomings in evaluating true expert capabilities. They predominantly rely on exam-style questions or probe information seeking rather than engaging models in authentic task-solving or open-ended generation. This closed-question paradigm failing to mirror the nature of real-world expert task-solving. 
% On the other hand, existing domain-specific benchmarks focus on isolated domains or tasks and their evaluation protocols can be misaligned with actual expert standards; for instance, some works \cite{bhambhoria2024evaluating} rely on general-purpose language model as a judge for evaluating LLMs' performance on domain-specific tasks without validating whether these automated judges are reliable on evaluating expert-level tasks. 

% To address these limitations, we introduce an open-ended benchmark accompanied by fine-grained evaluation rubrics that better reflect real-world expert demands and propose a decomposed-based automatic evaluation method to evaluate LLM performance on these tasks. 
% Specifically, our benchmark covers 11 expert-level tasks across 8 diverse domains—including law, material science, education, healthcare, chemistry, biology, medicine, and environment, social and governance— and center on expert-level applications that go beyond simple multiple-choice or knowledge-querying questions.
% % These tasks are grounded in realistic professional scenarios that require planning, synthesis, justification, and domain reasoning—capabilities essential for Expert AGI. % after failure model analysis 
% Each task is accompanied by a fine-grained evaluation rubric that better align with real-world expert needs. These rubrics not only support nuanced assessment of model outputs but also enable systematic meta-evaluation of LLM-as-a-judge approaches on expert-level tasks. To facilitate scalable evaluation, we further propose a decomposition-based automatic evaluation method, providing a straightforward yet reliable framework for assessing LLM performance across complex, open-ended expert scenarios.

% We evaluate 11 large language models on the proposed benchmark. Our key findings are summarized as follows: [TBD].
% In addition, we assess the reliability of existing LLM-as-a-judge methods in evaluating expert-level tasks, providing insights into their strengths and limitations in high-stakes, open-ended scenarios.

% Our goal is to push the boundaries of what LLMs can achieve by proposing benchmark and evaluation rubrics that better reflect the demands of real-world expertise.
% It is important to emphasize that our benchmark is not intended to serve as a comprehensive test for Expert AGI as excelling on it does not guarantee performance at the "90th percentile of skilled adults" across all domains. 
% However, we believe demonstrating strong performance on our benchmark is essential for Expert AGI, as it evidences both broad domain knowledge as well as robust task-solving capabilities in tackling a wide range of expert-level tasks.
% % However, we believe it should be necessary for Expert AGI to achieve strong performance on our proposed benchmark to show their comprehensive domain knowledge as well as robust task-solving capabilities across a wide range of expert-level scenarios. 
}

%% version 0

% Need of expert-level benchmark

% Large Language Models (LLMs) have demonstrated impressive capabilities in handling everyday tasks like answering general knowledge questions, writing emails, and summarizing text.
% As LLMs become increasingly integrated into various aspects of daily life, a natural question emerges: can they assist in tasks requiring expertise beyond general knowledge?
% % honestly i think we need to define "expert-level benchmark"
% Many real-world applications, such as scientific research, legal analysis, and medical decision-making, demand expert-level reasoning and knowledge synthesis beyond casual question-answering. 
% Addressing this gap requires rigorous evaluation through expert-level benchmarks that assess LLMs' capabilities in complex, high-stakes scenarios.

% Existing expert-level benchmark
% Not open-ended
% Not task-solving (application), but knowledge-querying
% Single-domain
% Evaluation might not align with expert


% Our benchmark tasks
% diverse domains
% expert task: expert-level applications beyond QA (multiple-choice / knowledge-querying open-ended QA), more align with expert needs


% Our evaluation
% rubrics: reflect expert needs, fine-grained 
% meta-evaluation of LLM-as-a-judge on expert-level tasks

% Benchmark experiments
% Model performance: coverage of rubrics item
% Evaluator performance: correlation with our results

